Doubly Robust Off-Policy Actor-Critic: Convergence and Optimality

Designing off-policy reinforcement learning algorithms is typically a very challenging task, because a desirable iteration update often involves an expectation over an on-policy distribution. Prior off-policy actor-critic (AC) algorithms have introduced a new critic that uses the density ratio for adjusting the distribution mismatch in order to stabilize the convergence, but at the cost of potentially introducing high biases due to the estimation errors of both the density ratio and value function. In this paper, we develop a doubly robust off-policy AC (DR-Off-PAC) for discounted MDP, which can take advantage of learned nuisance functions to reduce estimation errors. Moreover, DR-Off-PAC adopts a single timescale structure, in which both actor and critics are updated simultaneously with constant stepsize, and is thus more sample efficient than prior algorithms that adopt either two timescale or nested-loop structure. We study the finite-time convergence rate and characterize the sample complexity for DR-Off-PAC to attain an $\epsilon$-accurate optimal policy. We also show that the overall convergence of DR-Off-PAC is doubly robust to the approximation errors that depend only on the expressive power of approximation functions. To the best of our knowledge, our study establishes the first overall sample complexity analysis for a single time-scale off-policy AC algorithm.

==> algorithm.tex <==
\section{Doubly Robust Policy Gradient Estimator}
Doubly robust estimator has been widely used for off-policy evaluation of $J(w)$ \cite{tang2019doubly, jiang2016doubly}. Recently, \cite{kallus2020statistically} introduce the idea of doubly robust policy gradient estimator for averaged reward MDP.
Inspired by previous work, we propose a new policy gradient estimator in the infinity horizon discounted MDP setting, and further show that our new estimator of $\nabla J(w)$ enjoys a 3-way doubly robust property.

\subsection{Derivation of DR-PG}
First note that $J(w)$ has the following alternative form:
\begin{flalign*}
	J(w) = & (1-\gamma)\mE_{\mu_0}\big[V_{\pi_w}(s_0)\big] + \mE_d\big[\rho_{\pi_w}(s,a)(r(s,a,s^\prime) \nonumber\\
	&- Q_{\pi_w}(s,a) + \gamma \mE\big[V_{\pi_w}(s^\prime)|s,a\big])\big],
\end{flalign*}
where $\rho_{\pi_w}(s,a)=\nu_{\pi_w}(s,a)/d(s,a)$ is the {\em distribution correction ratio}. With a sample $(s_i, a_i, r_i, s^\prime_i)\sim \mcd_d$ and a sample $s_{0,i}\sim \mu_0$, we can formulate the following unbiased estimator of $J(w)$:
\begin{flalign*}
	\hat{J}(w) = & (1-\gamma)V_{\pi_w}(s_{0,i}) + \rho_{\pi_w}(s_i,a_i)(r(s_i,a_i,s^\prime_i) \nonumber\\
	&- Q_{\pi_w}(s_i,a_i) + \gamma V_{\pi_w}(s^\prime_i)).
\end{flalign*}
Note that $\nabla \hat{J}(w)$ is an unbiased estimator of $\nabla J(w)$ which takes the following form
\begin{flalign*}
	&\nabla_w\hat{J}(w) \nonumber\\
	&= (1-\gamma)d^v_{\pi_w}(s_{0,i}) + d^\rho_{\pi_w}(s_i,a_i)(r(s_i,a_i,s^\prime_i) \nonumber\\
	&- Q_{\pi_w}(s_i,a_i) + \gamma V_{\pi_w}(s^\prime_i)) \nonumber\\
	&+ \rho_{\pi_w}(s_i,a_i)(- d^q_{\pi_w}(s_i,a_i) + \gamma d^v_{\pi_w}(s^\prime_i)),
\end{flalign*}
where $d^v_{\pi_w}$, $d^q_{\pi_w}$, $d^\rho_{\pi_w}$ denote $\nabla_w V_{\pi_w}$, $\nabla_w Q_{\pi_w}$, $\nabla_w \rho_{\pi_w}$, respectively. By constructing nuisance estimators $\hat{Q}_{\pi_w}$, $\hat{\rho}_{\pi_w}$, $\hat{d}^\rho_{\pi_w}$ and $\hat{d}^q_{\pi_w}$, we can obtain the following policy gradient estimator
\begin{flalign}
	&G_{\text{DR}}(w) \nonumber\\
	&= (1-\gamma)\hat{d}^v_{\pi_w}(s_{0,i}) + \hat{d}^\rho_{\pi_w}(s_i,a_i)(r(s_i,a_i,s^\prime_i) \nonumber\\
	&- \hat{Q}_{\pi_w}(s_i,a_i) + \gamma \hat{V}_{\pi_w}(s^\prime_i)) \nonumber\\
	&+ \hat{\rho}_{\pi_w}(s_i,a_i)(- \hat{d}^q_{\pi_w}(s_i,a_i) + \gamma \hat{d}^v_{\pi_w}(s^\prime_i)),\label{dr_pg}
\end{flalign}
where $\hat{V}_{\pi_w}(s) = \mE_{\pi_w}[\hat{Q}_{\pi_w}(s,a)|s]$ and $\hat{d}^v_{\pi_w}(s) = \mE_{\pi_w}[\hat{Q}_{\pi_w}(s,a)\nabla_w\log\pi_w(s,a) + \hat{d}^q_{\pi_w}(s,a)]$. We then provide the following theorem to characterize the doubly robustness of $G_{\text{DR}}(w)$ .
\begin{theorem}[3-way Doubly Robustness]\label{thm1}
	Considering the policy gradient estimator in \cref{dr_pg}, we have
	\begin{flalign*}
		&\mE[G_{\text{DR}}(w)] - \nabla_w J(w)\nonumber\\
		&=-\mE[\varepsilon_{\rho}(s,a)\varepsilon_{d^q}(s,a)] - \mE[\varepsilon_{d^\rho}(s,a)\varepsilon_{q}(s,a)] \nonumber\\
		&\quad + \gamma\mE[\varepsilon_{\rho}(s,a)\varepsilon_{d^v}(s^\prime)] + \gamma\mE[\varepsilon_{\rho}(s,a)\varepsilon_{v}(s^\prime)],
	\end{flalign*}
	where the expectation is taken with respect to the randomness of sample (i.e., $(s,a,s^\prime)\sim\mcd_d$ and $s_0\sim\mu_0$) and $\varepsilon_{\rho}$, $\varepsilon_{q}$, $\varepsilon_{v}$, $\varepsilon_{d^\rho}$, $\varepsilon_{d^q}$, and $\varepsilon_{d^v}$ are errors of plug-in estimators defined as follows
	\begin{flalign*}
		&\varepsilon_{\rho} = \rho_{\pi_w}- \hat{\rho}_{\pi_w}, \quad \varepsilon_{q} = Q_{\pi_w} - \hat{Q}_{\pi_w},\quad \varepsilon_v = V_{\pi_w} - \hat{V}_{\pi_w},\nonumber\\
		&\varepsilon_{d^\rho} = d^\rho_{\pi_w}- \hat{d}^\rho_{\pi_w}, \quad \varepsilon_{d^q} = d^q_{\pi_w} - \hat{d}^q_{\pi_w},\quad \varepsilon_{d^v} = d^v_{\pi_w} - \hat{d}^v_{\pi_w}.
	\end{flalign*}
\end{theorem}
% ($\hat{\rho}_{\pi_w}=\rho_{\pi_w}$ and $\hat{d}^\rho_{\pi_w}=d^\rho_{\pi_w}$)
% ($\hat{Q}_{\pi_w}=Q_{\pi_w}$ and $\hat{d}^q_{\pi_w}=d^q_{\pi_w}$)
% ($\hat{\rho}_{\pi_w}=\rho_{\pi_w}$ and $\hat{Q}_{\pi_w}=Q_{\pi_w}$)
\Cref{thm1} shows that as long as (1) $\hat{\rho}_{\pi_w}$ and $\hat{d}^\rho_{\pi_w}$ are exact, or (2) $\hat{Q}_{\pi_w}$ and $\hat{d}^q_{\pi_w}$ are exact, or (3) $\hat{\rho}_{\pi_w}$ and $\hat{Q}_{\pi_w}$ are exact, our estimator $G_{\text{DR}}(w)$ is consistent, i.e., $\mE[G_{\text{DR}}(w)] - \nabla_w J(w)=0$.


